The metallicity dependence of the stellar initial mass function

Dust is important for star formation because it is the crucial component that couples gas to stellar radiation fields, allowing radiation feedback to influence gas fragmentation and thus the stellar initial mass function (IMF). Variations in dust abundance therefore provide a potential avenue by which variation in galaxy metallicity might affect the IMF. In this paper we present a series of radiation-magnetohydrodynamic simulations in which we vary the metallicity and thus the dust abundance from 1% of Solar to 3$\times$ Solar, spanning the range from the lowest metallicity dwarfs to the most metal-rich early-type galaxies found in the local Universe. We design the simulations to keep all dimensionless parameters constant so that the interaction between feedback and star-forming environments of varying surface density and metallicity is the only factor capable of breaking the symmetry between the simulations and modifying the IMF, allowing us to cleanly isolate and understand the effects of each environmental parameter. We find that at a fixed surface density more metal-rich clouds tend to form a slightly more bottom-heavy IMF than metal-poor ones, primarily because in metal-poor gas radiation feedback is able to propagate further, heating somewhat larger volumes of gas. However, shifts in IMF with metallicity at a fixed surface density are much smaller than shifts with surface density at fixed metallicity; metallicity-induced IMF variations are too small to explain the variations in mass-to-light ratio reported in galaxies of different mass and metallicity. We, therefore, conclude that metallicity variations are much less important than variations in surface density in driving changes in the IMF and that the latter rather than the former are most likely responsible for the IMF variations found in early-type galaxies.

==> scratch.tex <==
We use the adaptive mesh refinement code {\sc orion2} to carry out our simulations. The base numerical setup we use is identical to those of \citet{2014MNRAS.439.3420M} and \citet{2018MNRAS.476..771C}. For a detailed description of the setup, we refer the readers to the above-mentioned papers. 

{\sc orion2} uses \citep{2012ApJ...745..139L} to solve the equations of ideal magnetohydrodynamics coupled with self-gravity \citep{1998ApJ...495..821T, 1999ASSL..240..131K} and radiation transfer \citep{2007ApJ...656..959K} in the two-temperature, mixed-frame, grey, flux-limited diffusion approximation. The numerical methods we use are identical to those of \citet{2014MNRAS.439.3420M} and \citet{2018MNRAS.476..771C}, and we refer readers there for a more detailed description; here we merely summarise the key points. We use the {\sc orion2} adaptive mesh refinement (AMR) code \citep{Li21b} to carry out our simulations. The code uses the scheme of \cite{2012ApJ...745..139L} to solve the equations of ideal magnetohydrodynamics coupled to self-gravity \citep{1998ApJ...495..821T,1999ASSL..240..131K} and radiation transfer \citep{2007ApJ...656..959K} in the two-temperature, mixed-frame, grey, flux-limited diffusion approximation. We use the tabulated density- and temperature-dependent Rosseland- and Planck-mean opacities provided by \citet{Semenov03a}.

The code uses sink particles \citep{2004ApJ...611..399K} to replace regions where protostars are forming and that are collapsing beyond our ability to resolve. Each of these particles runs an instance of the one-zone protostellar evolution model described by \citet{2009ApJ...703..131O}, which prescribes the instantaneous properties (radius, luminosity, polytropic index, etc.) of the star that particle represents. The luminosity becomes a source term in our radiative transfer equations, and we also include feedback due to protostellar outflows via momentum sources around each sink particle. We use the outflow model described in \cite{2011ApJ...740..107C}: when mass is accreted onto a sink particle, a fraction $f_w$ of it is ejected back into the simulation in the form of an outflow, presumably from an unresolved inner disc. The outflow material is launched with a speed $v_w$. In our simulation, we use the same wind model parameters described in \cite{2012ApJ...747...22H} and \cite{2018MNRAS.476..771C}: $f_{w} =0.3$ and $v_w = \min(v_{\rm kep}, 60\;\mathrm{km/s})$, where $v_{\rm kep}$ is the Kepler speed at the surface of the protostar. These parameters are motivated by observations of the momentum budget of protostellar outflows \citep{2000prpl.conf..867R}. %(CITE: Richer et al., 2000, Protostars and Planets IV, pg. 867).

==> scratch_dcos.tex <==
shows the time evolution of the median and the 25th and 75th percentile ranges of the sink particle mass distributions for all the runs.



You need a paragraph here to discuss the recent Bate paper that focuses on the effects of the CMB. The approach I would take is just to note that we are doing somewhat different things than Bate is -- we are isolating one parameter at a time to do controlled experiments to understand it, while he is trying to replicate all the variations expected from high-redshift to today. I would just note here the difference in our findings, and explain that is why. Also note that the CMB will start to become a significant effect for us when it sets a temperature floor above the 10 K one we are using now; this occurs at z = 10/2.73-1 = 2.66.




The first time you refer to your paper in the text (presumably somewhere in the intro), write it as \citet[hereafter \citetalias{2022MNRAS.516.5712T}]{2022MNRAS.516.5712T}, which will render as Tanvir et al. (2022, hereafter Paper I}. Then use \citetalias{2022MNRAS.516.5712T} in all subsequent references to your paper.


There is a limitation to the radiation transfer method: we assume the dust and gas temperatures are equal. This is generally a good assumption for gas and dust temperature at densities above $\rm 10^{4}-10^{5} cm^{-3}$ \citep[e.g.,][]{2001ApJ...557..736G}. However, in the low-density regions, the density may be too low to allow efficient gas-dust coupling allowing gas to be either hotter or cooler than the dust. This is however unlikely to be a factor in determining the IMF since in regions where gas is collapsing and fragmenting, the density is high enough for gas and dust to be well coupled. Studies that have treated gas and dust temperatures separately \citep{Bate15a} find that its effect on fragmentation is minimal \citep{Bate19a}. 
